A General Framework for Distributed Partitioned Optimization

Decentralized optimization is widely used in large scale and privacy preserving machine learning and various distributed control and sensing systems. It is assumed that every agent in the network possesses a local objective function, and the nodes interact via a communication network. In the standard scenario, which is mostly studied in the literature, the local functions are dependent on a common set of variables, and, therefore, have to send the whole variable set at each communication round. In this work, we study a different problem statement, where each of the local functions held by the nodes depends only on some subset of the variables. Given a network, we build a general algorithm-independent framework for decentralized partitioned optimization that allows to construct algorithms with reduced communication load using a generalization of Laplacian matrix. Moreover, our framework allows to obtain algorithms with non-asymptotic convergence rates with explicit dependence on the parameters of the network, including accelerated and optimal first-order methods. We illustrate the efficacy of our approach on a synthetic example.

==> sections/experiments.tex <==
\section{Numerical simulations}

To illustrate the theoretical findings of Section \ref{sec:ring_of_cliques}, we carry out numerical simulations on synthetic data.

\ar{
\begin{itemize}
    \item Say about Linear Regression
    \item Describe the matrices $\A_i$ and vectors $b_i$ stored at the nodes
    \item Include plots
\end{itemize}
}
In this section, we present simulation results for solving a linear regression problem. 

In our case the linear regression problem is formulated as
$$\min_{\bx\in\R^{n}}~ F(\bx) = \frac{1}{m} \sum_{i=1}^m ||A_ix - b_i||^2_2$$

According to our constraints on minimization problem, we need to define matrices $A_i$ and vectors $b_i$ with knowledge about dependence of functions in every node from definite set of coordinates. That is, column of $A_i$ consists of zeros if $f_i$ does not depend on $i$th component and vice versa. $b_i$ can be arbitrary.

==> sections/problem_W_denotations.tex <==
\section{Problem with variable blocks}

\iffalse
\textbf{Notation}. Let $m$ be the number of nodes, $i, j$ -- indices of nods, $n$ is the number of all variables and $\ell$ -- index of coordinate. We also define $k$ as the size of clique. 
\fi


\subsection{New communication matrix}

Consider a minimization problem of type $\mathbb{R}$
\begin{align}\label{eq:problem_initial}
	\min_{x\in \R^n} \sum_{i=1}^m f_i(x^{\cN_i}).
\end{align}
Here each function $f_i$ depends on a subset of variables denoted by $\cN_i$ (we use notation $f_i(x^{\cN_i})$ for this). Further, we will write $f_i(x)$ but keep in mind that $f_i$ is dependent only on the subset $\cN_i$.

Each function is locally held by a separate computational node. Since functions are dependent only on subsets of variables, there is no need to exchange full vectors between them. Instead, for every variable $x^\ell$ we introduce a set of nodes that hold functions dependent on it: $\cV^\ell$ (i.e. $\cV^\ell = \braces{i:~ \ell\in\cN_i}$) and consider a communication network $\tilde\cG^\ell = (\cV^\ell, \cE^\ell)$, which we assume to be connected and undirected. Edge $(i, j)\in\cE^\ell$ if nodes $i$ and $j$ possess a common variable $x^\ell$ and can communicate this variable.

Let each node hold a local copy $x_i$ of variable vector and introduce stacked vector $\bx = [x_1^\top \ldots x_m^\top]^\top \in\R^{mn}$. Moreover, define $x^\ell = [x_1^\ell \ldots x_m^\ell]^\top\in\R^m$ to be the set of $\ell$-th vector components for $\ell = 1, \ldots, n$. We impose consensus constraints not on the whole vectors $x_i$ but only on common variables. That is, if the functions $f_i$ and $f_j$ have a common $\ell$-th coordinate dependent and $(i, j)\in\cG^\ell$, the corresponding constrain writes as $x_i^\ell = x_j^\ell$.
\begin{align*}
    \min_{\bx\in\R^{mn}}~ &F(\bx) = \sum_{i=1}^m f_i(x_i) \\
    \text{s.t.}~ &x_i^\ell = x_j^\ell~~ \forall (i, j)\in\cE^\ell,~ \ell = 1,\ldots, n.
\end{align*}


Let us rewrite the constraints using specific communication matrices associated with graphs $\braces{\cG^\ell}_{\ell=1}^n$. Given a network $\cV^\ell$, consider a matrix $\tilde W^\ell$ of size $|\cV^\ell|\times |\cV^\ell|$ which satisfies the following assumption.
\begin{assumption}
    Let $\cV^\ell = \braces{i_1^\ell, \ldots, i_{|\cV^\ell|}^\ell}$.
    \begin{itemize}
        \item $\tilde W^\ell$ is positive semi-definite.
        \item $\tilde W^\ell$ is symmetric.
        \item $\tilde W^\ell v = 0$ if and only if $v_{i_1^\ell} = \ldots = v_{i_{|\cV_\ell|}^\ell}$.
    \end{itemize}
\end{assumption}

After that, we define a communication matrix $W^\ell$ of size $m\times m$ that corresponds to the whole graph $\cG$.
\begin{align*}
    [W^\ell]_{ij} = 
    \begin{cases}
    [\tilde W^\ell]_{ij}, &\text{if}~ i, j\in \cV^\ell, \\
    0, &\text{else}.
    \end{cases}
\end{align*}


% Problem \eqref{eq:problem_initial} can be reformulated as
% \begin{align*}
%     \min_{\bx\in\R^{mn}} \sum_{k=1}^m f_i(x_i)~ \text{s.t. } W^1 x^1 = 0,~ \ldots,~ W^n x^n = 0.
% \end{align*}

Further, we can incorporate the constraints into one matrix $\mW$ associated with the set of networks $\braces{\cG^\ell}_{\ell=1}^n$. Denote $\be_\ell = (0\ldots 1\ldots 0)^\top\in\R^n$ the $\ell$-th coordinate vector and define
\begin{align}\label{eq:complex_lapl}
    \mW = \sum_{\ell=1}^n W^\ell \otimes \be_\ell \be_\ell^\top.
\end{align}



% For each $W^\ell$, denote its element in position $i, j$ as $w_{ij}^\ell$ and define
% \begin{align*}
%     \mW = 
%     \begin{bmatrix}
%         &w_{11}^1 & & & &w_{1m}^1 & & \\
%         & &\ddots & &\ldots & &\ddots & \\
%         & & &w_{11}^n & & & &w_{1m}^n \\
%         &\vdots &\vdots &\vdots &\ddots &\vdots &\vdots &\vdots \\
%         &w_{m1}^1 & & & &w_{mm}^1 & & \\
%         & &\ddots & &\ldots & &\ddots & \\
%         & & &w_{m1}^n & & & &w_{mm}^n \\
%     \end{bmatrix}.
% \end{align*}
According to the definition of $\bx$, we have $(W^\ell\otimes \be_\ell \be_\ell^\top)\bx = (W^\ell x^\ell)\otimes \be_\ell$ and $\mW\bx = \sum_{\ell=1}^m (W^\ell x^\ell)\otimes \be_\ell$.
%According to our definitions, we have $\bx = (x_1^1\ldots x_1^n~ x_2^1\ldots x_2^n \ldots x_m^1\ldots x_m^n)^\top$. Therefore, multiplication $\mW$ by $\bx$ writes as $\mW\bx = \cbraces{[W^1 x^1]^1 \ldots [W^n x^n]^1~ [W^1 x^1]^2 \ldots [W^n x^n]^2 \ldots [W^1 x^1]^m \ldots [W^n x^n]^m}^\top$, and communication constraints write as $\mW\bx = 0$. 
Communication constraints $\mW\bx = 0$ are equivalent to $\braces{W^\ell x^\ell = 0}_{\ell=1}^m$, and we obtain a reformulation that is standard for decentralized optimization
\begin{align}\label{eq:problem_affine_contraints}
    \min_{x\in\R^n}~ f(\bx) := \sum_{i=1}^m f_i(x_i)~ \text{ s.t. } \mW\bx = 0.
\end{align}
Any decentralized optimization algorithms including state-of-the-art primal (OPAPC \cite{kovalev2020optimal}) and dual (MSDA \cite{scaman2017optimal}) methods can be applied to the reformulated problem.


\subsection{Example}

Consider a graph $\cG = \cbraces{\cV, \cE}$, where $\cV = \braces{1, 2, 3}, \cE = \braces{(1, 2), (1, 3)}$, i.e. $\cG$ and let us have 2 coordinates. Let function $f_1$ be dependent on variables 1 and 2, $f_2$ be dependent only on variable 1 and $f_3$ be dependent only on variable 3. We build corresponding Laplacians for the variables 1 and 2 as follows.

\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.3\linewidth}
         \centering
         \includegraphics[width=0.6\linewidth]{figures/fullgraph.png}
         \caption{Full graph}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=0.6\linewidth]{figures/bluegreen.png}
         \caption{Subgraphs}
         \label{fig:three sin x}
     \end{subfigure}
        \caption{Graph $\cG$}
        \label{fig:three graphs}
\end{figure}

\begin{align*}
\blue{
\widetilde{W}^1 = 
\begin{bmatrix*}[c]
    &1&-1 \\
    &-1&1 \\
\end{bmatrix*}
}, \quad
\green{
\widetilde{W}^2 = 
\begin{bmatrix*}[r]
    &1&-1 \\
    &-1&1 \\
\end{bmatrix*}
}
\end{align*}
The corresponding Laplacians padded with additional zeros write as follows.
\begin{align*}
\blue{
W^1 = 
\begin{bmatrix*}[r]
    &1&-1&0 \\
    &-1&1&0 \\
    &0&0&0 \\
\end{bmatrix*}
},\quad
\green{
W^2 = 
\begin{bmatrix*}[r]
    &1&0&-1 \\
    &0&0&0 \\
    &-1&0&1 \\
\end{bmatrix*}
}
\end{align*}
According to \eqref{eq:complex_lapl}, we introduce matrix $\mW$:
\begin{align*}
\mW &= \blue{W^1}\otimes \be_1\be_1^\top + \green{W^2}\otimes \be_2 \be_2^\top \\
&= \blue{
\begin{bmatrix*}[r]
    &1&-1&0 \\
    &-1&1&0 \\
    &0&0&0 \\
\end{bmatrix*}
}\otimes
\begin{bmatrix*}[r]
    &1&0 \\
    &0&0
\end{bmatrix*} + 
\green{
\begin{bmatrix*}[r]
    &1&0&-1 \\
    &0&0&0 \\
    &-1&0&1 \\
\end{bmatrix*}
}\otimes
\begin{bmatrix*}[r]
    &0&0 \\
    &0&1
\end{bmatrix*} \\
&= 
\begin{bmatrix*}[r]
    &\blue{1} &0 &\blue{-1} &0 &\blue{0} &0 \\
    &0 &\green{1} &0 &\green{0} &0 &\green{-1} \\
    &\blue{-1} &0 &\blue{1} &0 &\blue{0} &0 \\
    &0 &\green{0} &0 &\green{0} &0 &\green{0} \\
    &\blue{0}&0&\blue{0}&0&\blue{0}&0 \\
    &0 &\green{-1} &0 &\green{0} &0 &\green{1} \\
\end{bmatrix*}
\end{align*}


On the other hand, the standard Laplacian for $\cG$ (without taking into account the different variables) writes as
\begin{eqnarray*}
W_{st} = 
\begin{bmatrix}
    &2&-1&1 \\ 
    &-1&1&0 \\ 
    &-1&0&1 \\ 
\end{bmatrix}
\end{eqnarray*}


\subsection{Spectrum of $\mW$}

We denote the set of \textit{unique} eigenvalues of matrix as $\bf{\Lambda}(\cdot)$.
\begin{lemma}\label{lemma:complex_lapl_spectrum}
    For matrix $\mW$ defined in \eqref{eq:complex_lapl} we have $\bLambda(\mW) = \bigcup\limits_{\ell=1}^n \bLambda(W^\ell)$.
    %$\ds\lambda_{\max}(\mW) = \max_{1\leq\ell\leq n} \lambda_{\max}(W^\ell)$ and $\ds\lambda_{\min}^+(\mW) = \min_{1\leq\ell\leq n} \lambda_{\min}^+(\mW)$
\end{lemma}
\begin{pf}
Firstly, let $\mW\bx = \lambda\bx$ for some $\bx\ne 0$ and $\lambda\in\mathbb{C}$. By definition of $\mW$, we have $W^\ell x^\ell = \lambda x^\ell$ for $\ell = 1, \ldots, n$. Since $\bx\ne 0$, there exists $\ell$ such that $x^\ell\neq 0$, and therefore $\lambda\in \bigcup\limits_{\ell=1}^n \bLambda(W^\ell)$.

Secondly, let $W^\ell x = \lambda x$ for some $\ell = 1, \ldots, n$. Setting $\bx = x^\ell\otimes \be_\ell$ we have 
$$
\mW\bx = \sum_{j=1}^n (W^\ell\otimes \be_j\be_j^\top)(x^\ell \otimes \be_\ell) = \sum_{j=1}^n (W^\ell x^\ell)\otimes (\be_j\be_j^\top \be_\ell) = (W^\ell x^\ell) \otimes \be_\ell = \lambda(x^\ell\otimes\be_\ell) = \lambda\bx
$$
i.e. $\lambda\in\bLambda(\mW)$. As a result, we get $\bLambda(\mW)\subseteq\bigcup\limits_{\ell=1}^n \bLambda(W^\ell)$ and $\bigcup\limits_{\ell=1}^n \bLambda(W^\ell)\subseteq \bLambda(\mW)$, therefore, $\bigcup\limits_{\ell=1}^n \bLambda(W^\ell) = \bLambda(\mW)$.
\end{pf}

It immediately follows from Lemma \ref{lemma:complex_lapl_spectrum} that $\ds\lambda_{\max}(\mW) = \max_{1\leq\ell\leq n} \lambda_{\max}(W^\ell)$ and $\ds\lambda_{\min}^+(\mW) = \min_{1\leq\ell\leq n} \lambda_{\min}^+(W^\ell)$. This gives an explicit formula for the condition number of $\mW$, that is, 
\begin{align*}
\chi(\mW) = \frac{\underset{1\leq\ell\leq n}{\max} \lambda_{\max}(W^\ell)}{\underset{1\leq\ell\leq n}{\min} \lambda_{\min}^+(W^\ell)}.
\end{align*}

% First, let us note that $\bf{\Lambda}(W^\ell) = \Lambda(\tilde W^\ell)\cup \braces{0, \ldots, 0}$ ($m - |\cV^\ell|$ zeros).

% By definition of $\mW$ it holds
% \begin{align*}
%     \norm{\mW\bx}_2^2 = \sum_{i=1}^n \norm{W^\ell x^{\ell}}_2^2
%     \leq \sum_{i=1}^n \lambda_{\max}(W^\ell) \norm{x^\ell}_2^2
%     \leq \max_\ell \lambda_{\max}(W^\ell) \norm{\bx}_2^2.
% \end{align*}
% In the above formula, the equality is reachable. Let $\ds\hat\ell = \argmax_\ell \lambda_{\max}(\tilde W^\ell)$, let $\hat x$ be the eigenvector corresponding to $\lambda_{\max}(\tilde W^{\hat\ell})$ and introduce $x_i = (0\ldots \hat x_i\ldots 0)^\top$ for $i = 1,\ldots,m$. Equality is attained at $\bx = (x_1^\top\ldots x_m^\top)^\top$. Therefore, $\ds\lambda_{\max}(\mW) = \max_\ell \lambda_{\max}(W^\ell)$.


